InstructVideo: Instructing Video Diffusion Models with Human Feedback

Diffusion models have emerged as the de facto paradigm for video generation. However, their reliance on web-scale data of varied quality often yields results that are visually unappealing and misaligned with the textual prompts. To tackle this problem, we propose InstructVideo to instruct text-to-video diffusion models with human feedback by reward fine-tuning. InstructVideo has two key ingredients: 1) To ameliorate the cost of reward fine-tuning induced by generating through the full DDIM sampling chain, we recast reward fine-tuning as editing. By leveraging the diffusion process to corrupt a sampled video, InstructVideo requires only partial inference of the DDIM sampling chain, reducing fine-tuning cost while improving fine-tuning efficiency. 2) To mitigate the absence of a dedicated video reward model for human preferences, we repurpose established image reward models, e.g., HPSv2. To this end, we propose Segmental Video Reward, a mechanism to provide reward signals based on segmental sparse sampling, and Temporally Attenuated Reward, a method that mitigates temporal modeling degradation during fine-tuning. Extensive experiments, both qualitative and quantitative, validate the practicality and efficacy of using image reward models in InstructVideo, significantly enhancing the visual quality of generated videos without compromising generalization capabilities. Code and models will be made publicly available.

==> figs/backup-intro.tex <==
\section{Introduction}
\label{sec:intro}

The emergence of diffusion models~\cite{sohl2015Diffusion_model,zhang2022gddim,ho2020denoising_DDPM,song2020score_generative_SDE} has significantly boosted the generative capabilities across various media content~\cite{wang2023modelscopeT2V,kong2021diffwave,ho2022video_diffusion_models,rombach2022stable_diffusion}.
% Generating videos, which is deemed challenging due to modeling high-dimensional data, benefits from this de facto generation paradigm~\cite{2023videocomposer,wang2023modelscopeT2V,blattmann2023align,ho2022video_diffusion_models,ho2022imagenvideo}, together with dataset scaling~\cite{singer2022make-a-video,wang2023lavie}.
This de facto generation paradigm has been proven beneficial for video generation~\cite{2023videocomposer,wang2023modelscopeT2V,blattmann2023align,ho2022video_diffusion_models,ho2022imagenvideo}, which is traditionally deemed challenging due to the complexity of high-dimensional data.
It thrives not only from diffusion models but also from the concurrent scaling of datasets~\cite{singer2022make-a-video,wang2023lavie}.
Despite the noticeable improvements brought by diffusion models, the visual quality of the resultant videos still leaves much room for enhancement~\cite{wang2023modelscopeT2V,wu2023tune-a-video}.
A significant contributing factor to this issue is the varying quality of web-scale data employed during the pre-training phase~\cite{Bain21Webvid,schuhmann2021laion}, thus resulting in a model capable of generating content that is visually unpleasing, toxic and misaligned with the prompt. 
% Although diffusion models are demonstrated effective in boosting generation quality, the goal of \textit{aligning generated videos with human preference} has never been researched, which has been studied in large language models~\cite{leike2018scalable_agent_align,askell2021general_language_alignment,ouyang2022InstructGPT,openai2023gpt4,touvron2023llama} and image generation~\cite{lee2023AlignT2I,xu2023ImageReward,wu2023HPSv1}.
% Although diffusion models are demonstrated effective in boosting generation quality, the visual quality of generated videos are still far from satisfaction~\cite{wang2023modelscopeT2V,wu2023tune-a-video}.
% The web-scale data utilized in the pre-training stage can contain data of various levels of quality~\cite{Bain21Webvid,schuhmann2021laion}, thus resulting in a model capable of generating content that is visually unpleasing, toxic and misaligned with the prompt.


% one of the popular paradigm 是offline policy。讲一下之前的offline policy是怎么做的
% 但是在Video generation里面用的话，会有问题。
% 1. 没有reward模型。
% 2. 计算量太大了（50步ddim）。language里面training和inference是align的，但是diffusion模型不是，所以导致计算量很大，image generation里面总是需要做一步生成。
%。   所以reformulate reward optimization成一个editting的问题。



\textit{Aligning generated videos with human preference} emerges as a potential solution to produce visually appealing videos, a notion that remains unexplored in video diffusion models. 
However, it has shown promising results in large language models~\cite{leike2018scalable_agent_align,askell2021general_language_alignment,ouyang2022InstructGPT,openai2023gpt4,touvron2023llama} and image generation~\cite{lee2023AlignT2I,xu2023ImageReward,wu2023HPSv1}.
Widely-adopted methods for aligning with human preference encompass off-line reinforcement learning (RL)~\cite{levine2020offlineRL,ouyang2022InstructGPT,black2023DDPO} and direct reward back-propagation~\cite{clark2023DRaFT,prabhudesai2023AlignProp}.
Typically, this involves a reward model trained on manually annotated datasets to subsequently fine-tune the pre-trained generative model.
Nevertheless, two major challenges persist in aligning video generation models with human preference:
\textbf{(i)} The curation of a sufficiently large annotated dataset to capture human preferences of videos labor-intensive, coupled with the computation- and memory-intensive demands of utilizing a ViT-H~\cite{wu2023HPSv2} or ViT-L~\cite{xu2023ImageReward} based video reward model.
% To understand the finer details, a A100 GPU can.
\textbf{(ii)} The optimization process geared towards human preference is computationally demanding, often requiring video generation from textual inputs. 
For a granular understanding, video generation pre-training using the DDPM~\cite{ho2020denoising_DDPM} objective demands a mere single inference step for every iteration while reward optimization requires a 50-step DDIM inference~\cite{zhang2022gddim}.


% One possible solution for generating visually pleasing videos is \textit{aligning generated videos with human preference}, which has never been researched in video diffusion models but studied and proven effective in large language models~\cite{leike2018scalable_agent_align,askell2021general_language_alignment,ouyang2022InstructGPT,openai2023gpt4,touvron2023llama} and image generation~\cite{lee2023AlignT2I,xu2023ImageReward,wu2023HPSv1}.
% Widely-adopted methods for aligning with human preference include off-line reinforcement learning (RL)~\cite{levine2020offlineRL,ouyang2022InstructGPT,black2023DDPO} and direct reward back-propagation~\cite{clark2023DRaFT,prabhudesai2023AlignProp}.
% Typically, a reward model is trained on manually-annotated datasets, and then utilized to fine-tune the pre-trained generative model.
% However, two major obstacles persist that hinders aligning a video generation model with human preference:
% \textbf{(i)} annotating a dataset large enough to reveal the human preference of videos is labor-intensive, and inferring a ViT-H~\cite{wu2023HPSv2} or ViT-L~\cite{xu2023ImageReward} based video reward model is computation-intensive;
% % prohibitatively large
% \textbf{(ii)} optimizing towards human preference usually requires generating the videos given text inputs, which is computation-intensive.
% % evaluate the whole video is computation-intensive.
% To be more specific, video generation pretraining using the DDPM~\cite{ho2020denoising_DDPM} objective requires only one step of inference while reward optimization requires 50-step DDIM inference~\cite{zhang2022gddim} for every iteration.
% % Although this paradigm proves effective 


To surmount the existing challenges, we propose \method, a model that efficiently instructs text-to-video diffusion models to follow human feedback. 
Regarding the challenge of lacking a reward model tailored for video generation, we postulate that the visual excellence of a video is tied to both the quality of its individual frames and the fluidity of motion across consecutive frames.
% Regarding the challenge of lacking a reward model tailored for video generation, we hypothesize that the visual quality of videos lies in the visual quality of frames and the motion quality between consecutive frames.
To this end, we resort to off-the-shelf image reward models, \textit{e.g.}, HPSv2~\cite{wu2023HPSv2}, to ascertain frame quality.
Drawing inspiration from temporal segment networks~\cite{wang2016TSN}, we propose Segmental Video Reward (SegVR), which strategically evaluates video quality based on a subset of sampled anchor frames.
% Drawing inspiration from temporal segment networks~\cite{wang2016TSN}, we evaluate generated videos by Segmental Video Reward (SegVR) that evaluates video quality on sampled anchor frames.
\textcolor{red}{SegVR offers dual benefits: it not only ameliorates computational burden but also prevents static video generation. (Need to be verified.)}
On the other hand, although LoRA~\cite{hu2021lora} is adopted by default to retain the capability to generate temporally smooth videos, SegVR still leads to videos with visual artifacts, such as structure twitching and color jittering.
Aiming to mitigate this, we propose Temporally Attenuated Reward (TAR), which operates under the hypothesis that central frames are afforded paramount importance, with the emphasis tapering off towards the peripheral frames.
% Aiming to mitigate this, we propose Temporally Attenuated Reward Fine-tuning (TARF), which is designed based on the hypothesis that central frames are afforded paramount importance, with the emphasis tapering off towards the peripheral frames.
This strategic allocation of importance across frames ensures a more stable and visually coherent video generation process.

% which put varying emphasis of frames during reward fine-tuning. 
% Reasons for twitching videos? (currently in methodology)
% 列出需要做的实验


% To surmount the existing challenges, we introduce \method, a robust model meticulously designed to seamlessly guide text-to-video diffusion models in sync with human feedback. Addressing the notable gap in reward models tailored for video generation, our framework postulates that the visual excellence of a video is intricately tied to both the quality of its individual frames and the fluidity of motion across successive frames. To this end, we leverage state-of-the-art image reward models, such as HPSv2~\cite{wu2023HPSv2}, to ascertain frame quality. Drawing inspiration from Temporal Segment Networks (TSN)~\cite{wang2016TSN}, we propose the Segmental Video Reward (SegVR) approach, which strategically evaluates video quality based on a subset of anchor frames. SegVR offers dual benefits: it significantly reduces computational overhead and \textcolor{red}{potentially} prevents the generation of static videos—assertions that we aim to empirically validate.

% However, despite its advantages, the default integration of LoRA~\cite{hu2021lora} in our model, intended to preserve video generation capabilities, occasionally results in visual artifacts such as structural twitching and color jittering in the generated videos. To mitigate these issues, we introduce Temporally Attenuated Reward Fine-tuning (TARF). TARF operates under the hypothesis that central frames hold a disproportionately higher importance, with this emphasis progressively diminishing as one moves towards the peripheral frames. This strategic allocation of importance across frames ensures a more stable and visually coherent video generation process, addressing the aforementioned visual inconsistencies.









Regarding the challenge of demanding reward fine-tuning caused by generating through the full DDIM sampling chain, we \textit{recast the problem of reward fine-tuning as an editing procedure}, leveraging the iterative refinement inherent to diffusion models during generation.
Within the established editing workflow using diffusion models~\cite{meng2021SDedit,couairon2022Diffedit,ceylan2023Pix2video,chai2023Stablevideo}, the primary visual content is initially corrupted by noise injection and subsequently manipulated guided by a target prompt.
% We \textit{reformulate reward fine-tuning as an editing procedure}, that refines the blurry and structural videos to more detailed and nuanced renderings, guided by human preference.
Drawing inspiration from them, we propose to progressively refine coarse, structural videos into detailed, nuanced renderings, instructed by human preferences.
Such blurry and structural videos, serving as the input foundation for reward fine-tuning, are procured by a straightforward diffusion process with negligible cost.
% generated by the first few steps of diffusion models
During generation, the optimized model retains the capability to produce videos directly from textual inputs.
In conjunction with gradient checkpointing~\cite{gruslys2016gradient_checkpointing} and back-propagation truncation of the sampling chain, we make reward fine-tuning on text-to-video diffusion models computationally attainable and effective.


A paragraph to summerize experiments and results.


% In addressing the challenge of intricate reward fine-tuning, we recast the reward optimization issue as an editing task, leveraging the iterative refinement inherent to diffusion models during generation. Within the established editing workflow using diffusion models~\cite{meng2021SDedit,couairon2022Diffedit,ceylan2023Pix2video,chai2023Stablevideo}, the primary visual content is initially subjected to noise, subsequently manipulated under the guidance of a target prompt. We \textit{envision reward fine-tuning as an editing process} that progressively refines coarse, structural videos into detailed, nuanced renderings, all steered by human preferences. These foundational, structural videos are procured via a straightforward diffusion process at minimal expense. Notably, during the generation phase, our enhanced model retains the capability to produce videos directly from textual inputs. In conjunction with gradient checkpointing~\cite{gruslys2016gradient_checkpointing} and truncation techniques, we make the task of reward fine-tuning in text-to-video diffusion models both feasible and impactful.







==> sec/abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

